Fine-grained Sentiment Controlled Text Generation

Controlled text generation techniques aim to regulate specific attributes (e.g. sentiment) while preserving the attribute independent content. The state-of-the-art approaches model the specified attribute as a structured or discrete representation while making the content representation independent of it to achieve a better control. However, disentangling the text representation into separate latent spaces overlooks complex dependencies between content and attribute, leading to generation of poorly constructed and not so meaningful sentences. Moreover, such an approach fails to provide a finer control on the degree of attribute change. To address these problems of controlled text generation, in this paper, we propose DE-VAE, a hierarchical framework which captures both information enriched entangled representation and attribute specific disentangled representation in different hierarchies. DE-VAE achieves better control of sentiment as an attribute while preserving the content by learning a suitable lossless transformation network from the disentangled sentiment space to the desired entangled representation. Through feature supervision on a single dimension of the disentangled representation, DE-VAE maps the variation of sentiment to a continuous space which helps in smoothly regulating sentiment from positive to negative and vice versa. Detailed experiments on three publicly available review datasets show the superiority of DE-VAE over recent state-of-the-art approaches.

==> 10Related.tex <==
\section{Related Work and Background}

There have been a flurry of works in the direction of text generation in recent years. Text generative models predominantly follow two distinct architectures (a)
Generative Adversarial Networks (GAN) ~\cite{zhang2016generating,kannan2017adversarial, zhang2016generating} that focus on generating text which mimics training data distributions, however they do not model any posterior distribution from the sentences, (b)  Variational Auto Encoders (VAE) \cite{bowman2015generating} which on the contrary model the posterior and is extended for conditional  text generation tasks including machine translation~\cite{bahdanau2014neural}, summerization ~\cite{li2017deep}, and dialog generation~\cite{kannan2017adversarial}. 


Controlled text generation gained momentum with the advent of the work ~\cite{hu2017toward}, where the authors have used sentiment as a controllable feature. However, there
is no evidence that the latent space would be disentangled by simply reconstructing a sentence from structured attribute representation augmented latent space. Other than sentiment, researchers have tried to generate text controlling  syntax  tree ~\cite{shi2016does}, topic ~\cite{wang2019topic} etc. However they are mostly focused on feature enriched text generation rather than controlling that feature.Text style transfer which primarily focuses on changing the style e.g sentiment or tense given a sentence could be termed as a subset of the controlled text generation problem. Several works ~\cite{shen2017style,zhang2018shaped,zhao2017adversarially} explore adversarial discriminators using parallel data for style transfer. Using non-parallel data and entangled representation the work ~\cite{wang2019controllable} achieves text-style transfer by editing the entangled latent representation until  the target attribute  is achieved. A recent work ~\cite{john2018disentangled} uses disentanglement using adversarial loss similar to ~\cite{hu2017toward}. However, none of them has \notetb{quantitatively} \noteng{Are we showing that??}  shown how much disentanglement they can achieve using their proposed methods.

Though achieving disentanglement in text representation is extremely challenging, disentangling latent space of image representation has been well explored in computer vision in recent years, and researchers have successfully disentangled the features (such as rotation and color) of images ~\cite{chen2016infogan, higgins2017beta}. In particular,
BetaVAE ~\cite{higgins2017beta} modifies Variational Autoencoder with a special emphasis to discover disentangled latent factors. However, over emphasis on the KL forcing disentanglement can cost the approximate posterior being insensitive of the observation. The paper  ~\cite{kumar2017variational} proposed a regularizer on the expectation of the approximate posterior for disentangled latent concepts. To provide a better tradeoff between disentanglement and reconstruction quality  ~\cite{kim2018disentangling}  proposed a method to factorize the representation to achieve disentanglement. These methods are unsupervised and works well in image dataset. 



Unlike the previous controlled text generative models, we propose
 ~\our{} which facilitates  the controlled text generation by obtaining a disentangled representation using  factorized prior like in the computer vision domain to achieve several benefits as described in the previous section. For this we propose a hierarchical architecture and feature supervision for attribute alignment in a desired dimension of the disentangled representation.


\noteng{I dont think we need an extra related work field, let us combine with intro}


\subsection{Brief of Hierarchical Variational Autoencoders} [Probably not needed]
Variational Autoencoders (VAE) \cite{kingma2013auto}, define a \textbf{decoding} probability distribution $p_\theta (x|z)$ to generate an observation $x$, given the latent variable $z$, that is sampled from a simple \textbf{prior} distribution $p_\pi(z)$. It learns an approximate probabilistic inference model $q_\phi(z|x)$ that \textbf{encodes} latent factors or features $z$ of the variation in the observed data~$x$ for optimizing the intractable marginal likelihood $\text{log } p_\theta(x)$.
General practice is to
maximize the expected lower bound of the likelihood on
observed data
\begin{align}
\max_{\phi,\theta}
\EE_{q_{\phi}(z | x)}\log p _{\theta}(x|z)-\text{KL}\bigl(q_\phi(z|x)||p_\pi(z)\bigr)
\label{eq:klobj}
\end{align}
To derive more complex features from a single input data-stream, %latent space,
multiple VAEs are stacked hierarchically \cite{rezende2014stochastic, sonderby2016ladder}.
For a hierarchical VAE with $\Lambda$ layers, the joint distribution of data and latent variables are modeled as below:
\begin{align*}
p(x, z_1, \dots, z_L) &= p(x | z_1) \textstyle
\prod_{\lambda=1}^{\Lambda-1} p_\theta(z_\lambda|z_{\lambda+1})  p_\pi(z_\Lambda)
\end{align*}
where $z_1$ is closest to $x$ and $z_\Lambda$ is the topmost layer. 
An increase in the number of layers, makes it difficult to capture any extra information in $z_\lambda$ in the higher layers. 


==> 30Training.tex <==
\section{Training Challenges}
\label{sec:posterior_collapse}
In general, VAE with autoregressive decoder while training with Eq.~\ref{eq:klobj} suffers from KL vanishing and posterior collapse.
It introduces two paths of information flow as depicted in Fig.~\ref{fig:paths} (b) at training time; in contrast with the one  which does not have any autoregressive decoder in Fig.~\ref{fig:paths} (a). If the information flows through the path B, potentially bypassing path A, the learned representation $z$ becomes exactly identical to
the prior. This happens when the powerful decoder (designed with LSTM)
starts neglecting the amortized inference network (encoder)
~\cite{he2019lagging,liu2019cyclical} and hence,
the $q_\phi$ starts to be equal to $p_\pi$, therefore
the KL vanishes quickly. If the prior does not have any semantic information about the input space; which is very common in practice for unsupervised generative models with a standard Gaussian prior,
 the learned posterior becomes a noise
 and the model collapses.
 On the contrary, a rich posterior distribution should capture the information of useful generative factors in a disentangled way.
 To enforce such disentanglement several approaches ~\cite{higgins2017beta} over-penalize
 the $KL$ loss in Eq.~\ref{eq:klobj} as
$
 \EE_{q_{\phi}(z | x)}\log p _{\theta}(x|z)-\beta\text{KL}\bigl(q_\phi(z|x)||p_\pi(z)\bigr).
 $
 Higher $\beta > 1$ is argued to encourage disentanglement at the cost of reconstruction error or likelihood in image datasets. However, high values of $\beta$, tries to pull $q_\phi(z|x)$ towards the prior heavily, causing  KL vanishing.
\begin{algorithm}[]
	\caption{Gated Periodic Update}
	\label{alg:main}
	\begin{footnotesize}
		\begin{algorithmic}[1]
			\STATE \texttt{/* Refer Figure~\ref{fig:paths} for path details*/}
			\STATE Input : $X = \{x^m_i\} \ i \in [0, \dots N], m \in [1,\dots,M], \eta $
			\STATE \texttt{/* Initialize encoder and decoder parameters */}
			\STATE $\phi, \theta \leftarrow \text{Initialize()}$
			\STATE $\Lcal = \Rcal + \Rcal_{pr} + KL$
			\STATE $\Ical \leftarrow $ CalculateMIConvergence()
			\REPEAT
			\IF{$\Ical$}
			\STATE  \texttt{/*Ordered layer update - Path C*/}
			\FOR {$i \in [0 \dots N]$}
			\STATE\texttt{/*Encoder Decoder update - Path A*/}
			\REPEAT
			\STATE $\xb$ $\leftarrow$ Random data minibatch
			\STATE $g_{\phi_i} \leftarrow \nabla_{\phi_i} \Rcal(\xb, \theta, \phi)$; $\phi_i \leftarrow \phi_i + \eta g_{\phi_i}  $
			\UNTIL{converges}
			\REPEAT 
			\STATE $\xb$ $\leftarrow$ Random data minibatch
			\STATE $g_{\theta_i} \leftarrow \nabla_{\theta_i} \Rcal(\xb, \theta, \phi)$; $\theta_i \leftarrow \theta_i + \eta g_{\theta_i} $
			\UNTIL{converges}
			\ENDFOR
			\STATE\texttt{/*Prior inference - Path D*/}
			\REPEAT
			\STATE $\xb$ $\leftarrow$ Random data minibatch
			\STATE $g_{\theta_{pr}} \leftarrow \nabla_{\theta_{pr}}$; $\theta_{pr} \leftarrow \theta_{pr} + \eta g_{\theta_{pr}}  \Rcal_{pr}(\xb, \theta)$ 
			\UNTIL{converges}
			\ELSE 
			\STATE  \texttt{/* Normal VAE Update - Path A, B, C*/}
			\FOR {$j \in [0,\dots,N]$}
			\STATE $i \leftarrow (N -j)$
			\STATE x $\leftarrow$ Random data minibatch
			\STATE $g_{\theta_i}, g_{\phi_i} \leftarrow \nabla_{\theta_i, \phi_i} \Lcal(\xb, \theta, \phi)$; 
			\STATE $\theta_i \leftarrow \theta_i + \eta g_{\theta_i} $; $\phi_i \leftarrow \phi_i + \eta g_{\phi_i} $
			\ENDFOR
			\ENDIF
			\UNTIL{converges}
		\end{algorithmic}
	\end{footnotesize}
\end{algorithm}
While conscious imposition of domain aware hierarchical prior in \our{} helps the model to learn a more expressive posterior from sequential data like text, this introduces another set of optimization challenges due to autoregressive decoder.
In the hierarchical set up, the model
introduces two more information flow paths as depicted by red paths (C and D) in Fig ~\ref{fig:paths} (c).
The approximate posterior distribution initially lags behind the true posterior ~\cite{he2019lagging}. As the posterior modeled in the upper layer of the hierarchy depends on the word layer posterior, it
not only lags behind the corresponding true feature posterior but also from the word layer's approximate posterior.  Similarly, once the feature posterior is obtained, we want to first model ``inferred prior" (path D), and then impose it on $z_0$ using $KL$.
Training the model, updating both the encoder and decoder simultaneously as formulated in  Eq.~\ref{eq:ob}, does not address this inference phase lag. 
However, we want to achieve, (a) high mutual information between observation and modeled representation, i.e., $I_q(z_0, x_0)$ and $I_q(z_i, x_i|z_0) \forall i > 0$  by maximizing the likelihood in Eq.~\ref{eq:w},~\ref{eq:f} , along with, (b) disentangled generative factors in the posterior distribution $q(z_0, x_0)$, which can be achieved by reducing KL between word posterior and inferred prior as Eq.~\ref{eq:kl_w},~\ref{eq:kl_f}. This trade-off between mutual information and KL can be maintained by an ordered update on parameters.


\subsection{Proposed Solution}
As described in Sec~\ref{sec:related}, several works propose different methods to mitigate the KL vanishing issue. In the direction of the annealing techniques, we combine Eq.~\ref{eq:w},~\ref{eq:f},~\ref{eq:kl_w} and~\ref{eq:kl_f} as: 
\begin{align*}
\label{eq:anneal1}
&\Rcal_{pr} + (1 - \alpha_w) I_q(x_0, z_0) + (1 - \alpha_f)\sum_{i=1}^{N} I_q(x_i, z_i | z_0) \\
&-\alpha_w \text{KL}(q_\phi(z_0)||p_\theta(z_0)) -\alpha_f\sum_{i=1}^N\ \text{KL} (q_{\phi}(z_{i}) || p_\pi(z_{i})) 
\end{align*}
where $\alpha_w$ and $\alpha_f$ are the annealing parameters. 
As described earlier, the feature layers' expressiveness is dependent on the word layer, hence, to facilitate the information flow through path C, we
propose a phase update by extending ~\cite{liu2019cyclical}. %Here
We introduced two annealing parameters, $\alpha_w$ and $\alpha_f$, for word layer and feature layer respectively, and we put a lag in their rise as
$\alpha_w = \text{tanh}\frac{(e \mod c)}{2}, \alpha_f = \text{max}\{0,\text{tanh}\frac{(e \mod c)- \gamma }{2}\} $, where $e$ is the current training epoch, $c$ is the cycle length, and $\gamma$ is the lag. We term this as \modcyc. However, this technique does not guarantee the ordered  parameter 
updates between the encoder and decoder, i.e., we first need to compute ``inferred priors" and then align the posterior $z_0$ with it, so that the variational update in the word encoder lags the decoder.
So, we propose a refined technique called \ourupdate{} 
 which regulates the parameter updates to achieve the desired performance.
It helps to initially increase the mutual information using aggressive autoencoder updates from bottom to top, followed by a variational update on encoder parameters in the reverse order, enforcing information flow through the paths C and D. The details are provided in Algorithm~\ref{alg:main}. CalculateMIConverge() checks if the mutual information has stopped increasing.


==> document1.tex <==
\iffalse
\subsection{Architecture Details}
\label{sec:architecture}

The number of topics a sentence can get associated with is a hyper-parameter $T$. Instead of a Gaussian Mixture Model, we derive $T$ different Gaussian representations from encoding  distribution as inferred prior for word sequences.  
For sentiments, we get
binary labels; which we encode in a latent space of size two,  finally the $p_\theta$  module transforms the encoded binary sentiments to a larger dimensional space.
We obtained best results by keeping the latent representation size for word sequences as 150.
We report the results with topic $T = 10$ and a latent variable of length fifteen for each of the topics.
We used pretrained fasttext word embedding vectors~\cite{mikolov2018advances} of length 300 and Adam Optimizer with learning rate of 0.005.
\fi
\section{Experimental evaluation}
In this section, we evaluate the performance of \our{} in terms of sentiment control using three different evaluation criteria -
%(a) accuracy of generating controlled attribute 
(a) sentiment control accuracy,
(b) fine tuning of sentiment, and (c) content preservation.
Additionally, we also discuss the
%we will show the interpretability power and 
extent of disentanglement in latent space $\zb_f$.
 
 \iffalse
 \begin{table}[]
 	\tiny
 	\centering
 	\begin{tabular}{l| l| l| l| l| l}
 	%	& \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Control \\ Generation\\ Accuracy\end{tabular}}  &\multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}} Degree of\\ control\end{tabular}}
\hline

&\begin{tabular}[c]{@{}l@{}}Control \\ Generation\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Degree of \\Control  \end{tabular}& \begin{tabular}[c]{@{}l@{}}Content \\ preservation\end{tabular} &
\begin{tabular}[c]{@{}l@{}}Disentanglement\end{tabular} &
\begin{tabular}[c]{@{}l@{}}Interpretability \end{tabular} \\
 		\hline
 		ctrlGen     & \checkmark &  & \checkmark &  &  \\
 		\hline
 		DVAE        & \checkmark &  & \checkmark &  &  \\
 		\hline
 		entangleGen & \checkmark &\checkmark  &\checkmark  &  &  \\
 		\hline
 		%betaVae     &  &  &  &  & \checkmark \\
 		%\hline
 		Our         &  \checkmark& \checkmark &  \checkmark& \checkmark & \checkmark\\
 		\hline
 	\end{tabular}
 \caption{Properties of different methods}
 \label{tab:baseline}
 \end{table}
\fi

 For our evaluation, 
 %We will demonstrate the results under these evaluation paradigms on 
 we rely on three large review datasets for sentiment controlled text generation - (a) \textbf{Yelp}~\cite{wang2019controllable} with $443248$, $2000$ and $1000$ number of labeled data on restaurant review for training, validation and test respectively with a vocabulary size of $9.5$K, (b) \textbf{Amazon}~\cite{wang2019controllable} with $554997$, $2000$ and $2000$ number of labeled data on product review for training, validation and test respectively with a vocabulary size $25$K, and (c) \textbf{IMDB}~\cite{diao2014jointly} movie review corpus which consists of $708929$, $4000$ and $2000$ number of unlabeled training, validation and test data with a vocabulary size of $28$K. This IMDB data has been tagged by Stanford sentiment tagger~\cite{socher2013recursive} and converted to three sentiment labels, namely, positive, neutral and negative. 

We compare the performance of \our{} with the following baselines that focuses on controlled text generation using disentanglement - %comprising of ensuring techniques:  
(a) \textbf{ctrlGen}~\cite{hu2017toward} which is a semi-supervised method for sentiment oriented text generation, and (b)~\textbf{DAE}~\cite{john2018disentangled} which is a supervised method that focuses on disentanglement using adversarial loss.
Other than these, we also compare \our{} with \textbf{entangleGen}~\cite{wang2019controllable} which focuses on text style transfer using entangled representation. Apart from these state-of-the-art baselines, we also use \textbf{DE-VAE-NR} (\our{} \textbf{N}on-\textbf{R}eversible transformation) as a baseline which is a variation of \our{}. In \textbf{DE-VAE-NR}, we replace the invertible normalizing flow used in \our{} with two neural networks designed as a two layer fully connected feedforward network responsible for capturing $q_\phi(\zb_f | \zb_s)$ and $p_\theta(\zb_s | \zb_f)$. 
%The capability of different competing methods are listed in Table ~\ref{tab:baseline} for easy comparison.
\begin{table}[]
	\small
	\centering
		\scalebox{0.8}{
	\begin{tabular}{c|c|c|c|c|c|c}
		\hline
		& \multicolumn{2}{c|}{Yelp} & \multicolumn{2}{l|}{Amazon} & \multicolumn{2}{l}{IMDB} \\ \hline
	%	&
	%	\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Control \\ Generation\\ Accuracy\end{tabular}} &
	%	\begin{tabular}[c]{@{}l@{}}Text style\\  transfer\\  Accuracy\end{tabular} &
	%	\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Control\\ Generation\\ Accuracy\end{tabular}} &
	%	\begin{tabular}[c]{@{}l@{}}Text style\\  transfer\\  Accuracy\end{tabular} &
	%	\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Control\\ Generation\\ Accuracy\end{tabular}} &
		%\begin{tabular}[c]{@{}l@{}}Text style\\  transfer\\  Accuracy\end{tabular} \\ \hline
		
		Methods &\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Control \\ Generation\end{tabular}} &
		\begin{tabular}[c]{@{}l@{}}Text style\\  transfer\end{tabular} &
		\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Control\\ Generation\end{tabular}} &
		\begin{tabular}[c]{@{}l@{}}Text style\\  transfer\end{tabular} &
		\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Control\\ Generation\end{tabular}} &
		\begin{tabular}[c]{@{}l@{}}Text style\\  transfer\end{tabular} \\ \hline
		%Methods     & Prior   & Post.   &   & Prior    & Post.   &    & Prior   & Post.   &   \\ \hline
		
		ctrlGen     &      0.72  &    0.70&         0.62             &0.63    &0.76                 &0.77   \\ \hline
		DAE         &    0.95        &  0.80   &   0.84   &   0.77 &    0.82         &  0.81 \\ \hline
		entangleGen &     -     &   \textbf{0.94} &     -        &  0.82   &    -         & 0.66  \\ \hline
		
		%$\beta$VAE     &      0.59   &  0.60           &   &          &             &    &         &             &   \\ \hline
		\hline
		\textbf{DE-VAE-NR} & 0.62       & 0.58   &          &    &    &   \\ \hline
		\our{}         &  \textbf{0.95}       & \textit{0.84}    &   \textbf{0.84}           &  \textbf{0.90}  &   \textbf{0.90}           & \textbf{0.86}  \\ \hline
	\end{tabular} }
	\caption{Sentiment control accuracy achieved by different methods. }
		%\our{} achieves the best score for all cases except text style transfer accuracy for Yelp}.
	\label{tab:sentiment}
\end{table}
\subsection{Sentiment Control Accuracy}
%\subsection{Accuracy of attribute controlled Text Generation}
Here we measure the quality of sentiment control by quantitatively evaluating the sentiment oriented sentence generation accuracy.
%generating sentences with designated sentiment. 
For this purpose, we train a sentiment classifier by extending \textbf{BERT}~\cite{devlin2018bert}. This classifier is $95\%$ accurate on Yelp data and $85\%$ accurate on Amazon and IMDB data
 %on validation data 
% after training with a tagged training set,
 which demonstrates its robustness. 
Specifically, \our{} generates sentences by regulating the values in the designated dimension of $\zb_f$ which is modeled to control the sentiment; we use the pre-trained sentiment classifier to assign sentiment labels to the generated sentences. Similarly, we generate sentences using the baseline methods.
We report the accuracy of sentiment oriented sentence generation 
%regulating $\zb_f$ 
in two different ways - (a) \textbf{Control generation accuracy} which is accuracy of generating sentences where the generative representation is sampled from the prior (i.e. from $p_\pi(\zb_f)$ in case of \our{}), followed by assigning the desired value for the sentiment representation (i.e. $\zb_a$ for \our{}), and
%(b) posterior - when the representation is sampled from the posterior distribution of test sentences and trying to convert to positive or negative 
(b)  \textbf{Text style transfer accuracy} which is accuracy of generating sentences with opposite polarity sentiment from posterior distribution of a sentence $x$, given the posterior distribution of $x$ bearing a specific type of sentiment.
%sampled both from prior and posterior distribution in 

From the results reported in Table~\ref{tab:sentiment}, it can be observed that \our{} outperforms all competing methods across all datasets for controlled text generation, other than text style transfer accuracy in case of Yelp. 
The superior performance of \our{} stems from the fact that it learns a disentangled feature representation where sentiment information is modeled in a single dimension which is independent of other dimensions. So, regulating the sentiment value along this designated dimension gives better control while generating sentences bearing the same sentiment. %generation.
%which bear the same sentiment.
%The superior performance of our method is due to its ability to align sentiment with the designated dimension using feature supervision and further making it independent to other dimensions in $\zb_f$. 
Further, in case of \textbf{DE-VAE-NR}, we train the parameters of the transformation network by maximizing the likelihood of $\zb_s$ as $\EE_{q_\theta}p_\theta(\zb_s | \zb_f)$ such that the minimum KL between $q_\phi(\zb_f | \zb_s)$ and $p_\theta(\zb_s | \zb_f)$ is found to be in the range $0.02-X$ across all datasets; however, the performance of \textbf{DE-VAE-NR} is significantly low compared to \our{} which shows the significance of using invertible normalizing flow. Close inspection reveals that even though the KL was low, as the decoded distribution $\zb_s$ was not exactly the same as the encoded distribution, it was generating sentences  different from the original sentence. This shows the importance of invertible normalizing flow as a design choice. 
The closest competitor to our method is \textbf{DAE} for controlled text generation with comparable performance to \our{}. 
%In fact, it performs comparably to \our{} in case of Yelp and Amazon. 
The reason is that \textbf{DAE} achieves disentanglement between style space and content space using extensive adversarial training and incorporates auxiliary multi-task loss for sentiment or style.
 %in content and style space, 
 %however, this does not always guarantee the disentanglement.  
 Further, in comparison to other methods, \textbf{ctrlGen} performs poorly for controlled text generation. 
 %since it tries to achieve disentanglement by making the sentence representation independent of structured representation of sentiment which is externally provided. 
 We speculate that \textbf{ctrlGen} has comparatively less control than other methods since it does not model feature representation from sentence representation and tries to control generation by providing only a one hot encoding of sentiment externally.
\iffalse
make  externally provided sentiment representation, it is hard to achieve a sentence representation insensitive of the sentiment. Hence in comparison to other methods it performs poorly.
 %suffers from similar issues and hence it performs similar to \textbf{DAE}.
 % On the other hand, though $\beta$VAE focuses in achieving disentanglement by making the dimensions independent with each other, it cannot guarantee that only a single dimension will be responsible for sentiment variation without explicit feature supervision. As identification of a single dimension responsible for variation of the sentiment is non-trivial, $\beta$VAE performs the worst among competing methods. 
  \fi
  We have reported the accuracy of \textbf{entangleGen} only for text style transfer in Table~\ref{tab:sentiment} since it focuses only on attribute transfer. We observe that \textbf{entangleGen} achieves better accuracy on Yelp dataset than our method; however, \our{} performs superiorly on all other datasets.
  %in the  performance is poor in IMDB which has three sentiment labels. 
  %The architecture used by 
  Since \textbf{entangleGen} inherently supports binary-valued attributes by design,
 %As \textbf{entangleGen} is designed for text style transfer 
 it can modify the sentiment value towards its opposite polarity only using Fast-Gradient-Iterative-Modification. 
 %of a given sentiment value, 
Hence, its performance suffers in IMDB data where there are more than two sentiment values. 
%as is the case for IMDB data. 

%Here, we have extended this analysis for style transfer which considers change in sentiment polarity of the examples i.e. positive to negative and vice-versa. We can see that \our{} performs comparably to \textbf{entangleGen} while outperforming others.


 
\iffalse
 \begin{table}[]
 	\small
 	\centering
 	\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
 		\hline
 		& \multicolumn{3}{c|}{Yelp} & \multicolumn{3}{l|}{Amazon} & \multicolumn{3}{l}{IMDB} \\ \hline
 		&
 		\multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Control \\ Generation\\ Accuracy\end{tabular}} &
 		\begin{tabular}[c]{@{}l@{}}Text style\\  transfer\\  Accuracy\end{tabular} &
 		\multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Control\\ Generation\\ Accuracy\end{tabular}} &
 		\begin{tabular}[c]{@{}l@{}}Text style\\  transfer\\  Accuracy\end{tabular} &
 		\multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Control\\ Generation\\ Accuracy\end{tabular}} &
 		\begin{tabular}[c]{@{}l@{}}Text style\\  transfer\\  Accuracy\end{tabular} \\ \hline
 		Methods     & Prior   & Post.   &   & Prior    & Post.   &    & Prior   & Post.   &   \\ \hline
 		
 		ctrlGen     &      0.72   &   0.77  &    0.70&         0.62 &0.62             &0.63    &0.76         &     0.77        &0.77   \\ \hline
 		entangleGen &     -    &      - &   0.94 &     -     &       -      &  0.45  &      -   &    -         & 0.66  \\ \hline
 		DAE         &    0.95     &     -     &  0.89   &   0.84 &    -    &   0.77 &    0.82     &             &  0.77 \\ \hline
 		%$\beta$VAE     &      0.59   &  0.60           &   &          &             &    &         &             &   \\ \hline
 		Our         &  \textbf{0.95}       & \textbf{0.84}  & \textit{0.84}  &   \textbf{0.84}       &       \textbf{0.77}     &  \textbf{0.90}  &   \textbf{0.90}     &       \textbf{0.77}      & \textbf{0.86}  \\ \hline
 	\end{tabular}
 \caption{Results on control text generation accuracy and text style transfer. }
 \label{tab:sentiment}
\end{table}
\fi
\begin{figure}[!t]
	\vspace{-4mm}
	\centering
		\hspace*{-0.55 cm}
		\includegraphics[width=0.40\textwidth, clip]{figure/legend}\\
	\hspace*{-0.55 cm}
	\subfloat[Yelp (Positive) ]{\includegraphics[width=0.25\textwidth, clip]{figure/yelp_pn_new1.png}}
	\hspace*{-0.3 cm}
	\subfloat[Amazon (Positive)]{\includegraphics[width=0.25\textwidth, clip]{figure/amazon_pn_new1.png}}
	\hspace*{-0.4 cm}
	\subfloat[Yelp (Negative)]{\includegraphics[width=0.25\textwidth, clip]{figure/yelp_np_new1.png}}	
	\hspace*{-0.3 cm}
	\subfloat[Amazon (Negative)]{\includegraphics[width=0.25\textwidth, clip]{figure/amazon_np_new1.png}}\\
	\hspace*{-0.55 cm}
	\subfloat[Yelp (Positive)]{\includegraphics[width=0.25\textwidth, clip]{figure/ov_yelp_pn_new.png}}
	\hspace*{-0.3 cm}
	\subfloat[Amazon (Positive)]{\includegraphics[width=0.25\textwidth, clip]{figure/ov_amazon_pn_new.png}}
	\hspace*{-0.4 cm}
	\subfloat[Yelp (Negative)]{\includegraphics[width=0.25\textwidth, clip]{figure/ov_yelp_np_new.png}}	
	\hspace*{-0.3 cm}
	\subfloat[Amazon (Negative)]{\includegraphics[width=0.25\textwidth, clip]{figure/ov_amazon_np_new.png}}
	\caption{Upper row denotes variation of average sentiment score of generated sentences with fine-tuned degree of sentiment control. Bottom row indicates variation of  Jaccard score of generated sentences with fine-tuned degree of sentiment control. The original sentence sentiment is indicated in brackets.
	}
	\vspace*{-0.2cm}
	\label{fig:labelvariation}
\end{figure}
\subsection{Fine tuning of sentiment and Content preservation}
In this section, we discuss the performance of \our{} in terms of both the evaluation criteria - fine tuning of sentiment and content preservation. 
%five different levels of sentiment given a sentence. 
As by design, \our{} is able to capture the entire behaviour of the sentiment in a continuous latent space of a single dimension, we first estimate the maximum value $f_{max}$ and minimum value $f_{min}$ of this dimension from training data.
Then we use this range and
%first the range of the values from the validation set and 
interpolate between $f_{max}$and $f_{min}$ in $20$ different bins where the value of $i^{th}$ bin ($1\leq i\leq 20$) is denoted as $f_{min} + \frac{(f_{max} - f_{min}) i}{20}$. Given a feature representation $\zb_f$ corresponding to a sentence $\xb$, we assign a bin value to $\zb_a$ (last dimension of $\zb_f$) and sample $100$ sentences corresponding to this modified $\zb_a$. We repeat this procedure
%of $\zb_a$ for $100$ sampled sentences 
corresponding to each bin value. 
Similarly, we extend \textbf{ctrlGen} to generate sentences by interpolating $20$ different values sampled from the range $[0,1]$ for the structured two-dimensional sentiment representation.
% such that the summation of these values equals one.
%$[0,1]$ in the designated two dimensions for sentiment. 
%In contrast to our model, other state-of-the-art methods for controllability (eg. 
As \textbf{entangleGen} can only regulate the sentiment of the given sentence in the opposite polarity
%i.e. positive to negative or vice-versa 
using $35$ different degrees of sentiment, 
%We use five different degrees of change as described in \textbf{entangleGen}, to control the degree of sentiment in one direction. 
we have aggregated them within ten bins. It may be noted that we have excluded \textbf{DAE} from this evaluation since it models sentiment in a multi-dimensional space and fine tuning sentiment in such a space is non-trivial. Additionally, we have also excluded comparison with \textbf{DE-VAE-NR} due to its poor performance on sentiment control.   

To quantitatively measure the performance of fine tuning of sentiment, we have used the pre-trained Stanford sentiment regressor~\cite{socher2013recursive} which provides sentiment scores of sentences generated for \our{} and other methods between $[0,1]$ with $1$ denoting most positive and $0$ denoting most negative. 
%The sentences generated by \our{} and other methods are scored by this pre-trained model. 
Further, we evaluate the model performance in terms of content preservation while fine tuning sentiment. For this purpose, we compute \emph{Jaccard overlap}~\cite{tustison2009introducing} of unigram words in the original sentence  $x$ and the generated sentence $y$, computed as $\frac{|w_x \cap w_y|}{|w_x \cup w_y|}$, where $w_{.}$ denotes the set of words after excluding stopwords in corresponding sentence. 
%while calculating the same. 
%generated scores.
%and calculated the sentiment scores using the pre-trained model. 

In Figure~\ref{fig:labelvariation}, we have demonstrated the variation of mean sentiment scores (Figure~\ref{fig:labelvariation}(a)-(d)) and \emph{Jaccard overlap} scores (Figure~\ref{fig:labelvariation}(e)-(h)) in different bins (with $1$ denoting most negative and $20$ denoting most positive control signal).
We separately show the variations of mean positive (negative) sentiment value over the different bins when starting sentiment was negative (positive).
% sentiment positive and similarly for negative.
%sentence we show how the average neragive score of the sentences are varying and for negative sentiment start sentence we show the opposite.
%in these fine tuned sentiment buckets for both positive and negative start sentence. 
%From sub-figure (a), (b) it can be easily seen that \our{} achieves 
%As \textbf{entangleGen} can regulate only opposite polarity, it occupies the half spectrum of each image.
We can observe from Figure~\ref{fig:labelvariation}(a) that the sentiment scores vary over a large range ($0.17$) between the first and last bins for \our{} in case of Yelp when the original sentence is positive; however, \textbf{entangleGen} can achieve a greater negative sentiment score for bins $1-4$. In comparison to these methods, \textbf{ctrlGen} shows a very small drift ($0.1$) in sentiment scores over all the bins with almost zero variation for bins $13-20$.   
%consistently generates sentences with higher negative sentiment scores over all the bins.
This implies that \textbf{ctrlGen} has lesser control in fine tuning sentiment scores over the bins compared to \our{}. Interestingly, if we check the corresponding variation of \emph{Jaccard overlap} in Figure~\ref{fig:labelvariation}(e), we find that the sentences generated by \textbf{ctrlGen} while fine tuning sentiment performs poorly in terms of preserving content. 
%despite generating negative sentences with higher negative sentiment scores. 
For \textbf{entangleGen}, the \emph{Jaccard overlap} is high only for the bins $6-8$. %This indicates \textbf{ctrlGen} is losing content while trying to generate negative sentences with larger  negative values. 
On the other-hand, the \emph{Jaccard overlap} scores are high for \our{} over all the bins demonstrating its effectiveness in content preservation while fine tuning sentiment. 
%It shows a tendency of rise and drops a bit in bins < 5. In contrast \textbf{entangleGen} shows an initial drift in rise but drops heavily after that. 
%getting higher in bins less than 10 than the rest. When \our{} tries to model more positive sentences starting with existing positive sentence, it picks up more words to emphasis on the sentiment which lowers the jaccard score.

In case of Amazon data, Figure~\ref{fig:labelvariation}(b) shows that we can easily achieve a smooth variation in the negative sentiment scores for \our{} with a very high drift of $0.08$ between the first and last bins. Compared to \our{}, \textbf{ctrlGen} shows negligible drift for bins $11-20$. Figure~\ref{fig:labelvariation}(b) also shows that \textbf{entangleGen} performs poorly in fine tuning sentiment for Amazon. Looking into the corresponding \emph{Jaccard overlap} scores in Figure~\ref{fig:labelvariation}(f), it can be easily observed that \our{} achieves higher \emph{Jaccard overlap} scores compared to other methods with low scores only for last few bins. Similar observation holds true for the opposite case when the original sentence is negative across all datasets as evident from Figures~\ref{fig:labelvariation}(c)-{(d) and Figures~\ref{fig:labelvariation}(g)-(h). This signifies the fact that \our{} can achieve a superior fine tuning of sentiment while preserving the content of generated sentences compared to the state-of-the-art methods. Since we could not observe any significant variation in sentiment scores of generated sentences for IMDB over different bins for any of the  methods, we have not discussed these results for IMDB dataset. 
%as this datasets sentences sentiment bearing score is low. Hence variations are not prominent in any of the methods. 
%starting fro extremely positive to negative. The performance superiority is due to the fact that \our{} can regulate the same.

Further, we have sampled an original sentence from data and have shown the corresponding generated sentences using \our{} for different bins in Table~\ref{tab:example}. 
As evident from this table, we are able to preserve the content and semantics of the original sentence while still observing a smooth interpolation in the degree of sentiment transfer.
% as shown in Figure~\ref{fig:labelvariation}. 
An interesting observation here is that though the exact word overlap is low for generated sentences with very high sentiment scores (e.g. in case of bins $1$ and $20$ in Table~\ref{tab:example}), it is semantically similar to the original sentence which is also exemplified by the results shown in Figure~\ref{fig:labelvariation}.


%that \our{} can smoothly control the degree of sentiment transfer in both the directions i.e. given a sentence of positive sentiment, we can regulate it in such a way that it can be converted to extreme positive as well as to extreme negative. The degree of control of \textbf{entangleGen} in one direction is similar to our method. However, \textbf{ctrlGen} performs poorly. 

%From the Table~\ref{tab:interpolation} it can be seen that thou

%We calculate the score of the sampled sentences in these buckets and observe that the scores interpolate smoothly. 


% Please add the following required packages to your document preamble:
% \usepackage{multirow}


%As discussed in the previous section, we are observing a smooth interpolation in sentiment while still preserving the overall content as evident from this table.
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
	\small
	%\centering
	
	\scalebox{0.85}{
	\begin{tabular}{l|l|l}
		\hline
		Bins& Original Sentence - Positive                                             & Original Sentence - Negative                           \\ \hline
		original & i ' m very impressed with the level of \textcolor{blue}{care} here !              & but their \textcolor{blue}{inventory} was questionable !      \\ \hline
		b=1   & i am \textbf{totally disappointed} by the help  \textbf{completely not} \textcolor{blue}{caring} .         & but their customer service was \textbf{impeccable} ! \\ \hline
		b=5    & i am \textbf{totally disappointed} with the compassion ( \textbf{not} \textcolor{blue}{caring} ) .         & but their was \textcolor{blue}{inventory} was \textbf{ridiculous} ! \\ \hline
		b=10     & i am \textbf{totally disappointed} by the owners ... \textbf{not} \textcolor{blue}{caring} . & but their \textcolor{blue}{inventory} was \textbf{awful} !         \\ \hline
		b=13     & i am \textbf{not totally disappointed} by the \textcolor{blue}{caring} staff !             & but their \textcolor{blue}{inventory} was \textbf{empty} !             \\ \hline
		b=16     & i am \textbf{highly recommend}  - this resort \textbf{truly\textcolor{blue}{ care}} !   & their \textcolor{blue}{inventory} was \textbf{ impressive} !            \\ \hline
		b = 20 & i am \textbf{truly kind of `impressed' }- oh \textbf{highly recommend} this staff ! & their selection was \textbf{outstanding} !        \\ \hline
	\end{tabular}}
\caption{Fine grained sentiment control of sentences from extreme negative to extreme positive. \textbf{Bold} letters indicates words with sentiment and the color \textcolor{blue}{blue } indicates important words to be preserved.}
	\label{tab:example}
\end{table}
\subsection{Model Ablation Study}
\iffalse
In this section, we perform an ablation study for highlighting the benefits of design choices for the transformation network followed by the evidence of sentiment control achieved by modifying $\zb_a$.
%Here we discuss two things (a) the effectiveness showing  and (b) the  information.
As discussed in Section~\ref{sec:model}, the performance of the hierarchical architecture of \our{} is highly dependent on the choice of the transformation network. We replace the invertible normalizing flow used in \our{} with two neural networks responsible for capturing $q_\phi(\zb_f | \zb_s)$ and $p_\theta(\zb_s | \zb_f)$. Each of them is designed as a two layer fully connected feedforward network. We train the parameters of this transformation network by maximizing the likelihood of $\zb_s$ as $\EE_{q_\theta}p_\theta(\zb_s | \zb_f)$. The minimum KL between $q_\phi(\zb_f | \zb_s)$ and $p_\theta(\zb_s | \zb_f)$ is found to be as low as $0.02$; however, the performance of this model variation on Yelp dataset for text style transfer accuracy drops to $58\%$ from $84\%$ achieved using invertible normalizing flow. Close inspection reveals that even though the KL was low, as the decoded distribution $\zb_s$ was not exactly the same as the encoded distribution, it was generating sentences  different from the original sentence. This shows the importance of invertible normalizing flow as a design choice. 
%\subsection{Disentanglement  and Interpretability Analysis}
\fi
Here we perform an ablation study by demonstrating the importance of the last dimension $\zb_a$ of the representation $\zb_f$ in capturing sentiment. As we ensure independence of every dimension, we calculate the correlation of every dimension of $\zb_f$ with the sentiment labels in test data. We observe that $\zb_a$ achieves the highest correlation of $0.72$ in Yelp and $0.42$ in Amazon. We further train a logistic regression classifier with $\zb_a$ of training data as a feature to predict sentiment labels, and we achieve a high accuracy of $0.85$ and $0.64$ on test data in Yelp and Amazon respectively. While training with the most correlated dimension of $\zb_f$ other than $\zb_a$ with correlation $0.12$ for Yelp and $0.14$ for Amazon, we achieve an accuracy of only $0.52$ and $0.58$ respectively. This implies that $\zb_a$ is the most expressive dimension for capturing sentiment.




\iffalse
Here we analyse the extent to which we are able to achieve disentanglement of the latent space and subsequently show the model interpretability.
%Here we focus on some quantitative measures to calculate the disentanglement of the latent space.
%We analyze how the style (sentiment) and content of the latent space are disentangled.
First we aim to qualitatively understand how the latent space is disentangled. For this purpose, we use  the validation set data and generate their latent  disentangled representation $\zb_f$. Then we use t-SNE~\cite{maaten2008visualizing} to plot the representation of  $u_f$ (see sec.~\ref{sec:model})and $\zb_a$ which is the last dimension of $z^*$. In Fig.~\ref{TBD}, we can see that the different sentiments get distinguishably separated by the last dimension in the latent space whereas they are overlapping when using the remaining dimensions denoted by $u_f$. 

To further verify the same quantitatively, we adopt the technique proposed by \textbf{DAE}~\cite{john2018disentangled}. We train a classifier with the representation of $u_f$ and predict the sentiment. It can be seen that just by using a threshold approach on the last dimension of $z^*$ i.e. $z_f^1$, we get much better accuracy compared to using $u_f$. 
These results verify the effectiveness of \our{}  in achieving disentanglement to a great extent. In comparison to \our{}, \textbf{ctrlGen} and \textbf{DAE} performs poor disentanglement as their classification accuracy based on the non-style space is much higher than \our{}, implying that there is some style information hidden in the non-style space for \textbf{ctrlGen} and \textbf{DAE}. 
\fi
% whereas the content space does not.

%We see the 128-dimensional content vector c is not particularly discriminative for style. Its accu- racy is slightly better than majority guess. How- ever, the 8-dimensional style vector s, despite its low dimensionality, achieves substantially higher style classification accuracy. When combining content and style vectors, we observe no further improvement. 


%\section{Model ablation study}

%\xhdr{Effect of control flow}






 










